An $\tilde\Omega\big(\sqrt{\log |T|}\big)$ Lower Bound for Steiner Point Removal

In the Steiner point removal (SPR) problem, we are given a (weighted) graph $G$ and a subset $T$ of its vertices called terminals, and the goal is to compute a (weighted) graph $H$ on $T$ that is a minor of $G$, such that the distance between every pair of terminals is preserved to within some small multiplicative factor, that is called the stretch of $H$. It has been shown that on general graphs we can achieve stretch $O(\log |T|)$ [Filtser, 2018]. On the other hand, the best-known stretch lower bound is $8$ [Chan-Xia-Konjevod-Richa, 2006], which holds even for trees. In this work, we show an improved lower bound of $\tilde\Omega\big(\sqrt{\log |T|}\big)$.

==> construction.tex <==
\section{Proof of \Cref{thm: main}}

The hard instance is constructed as follows.
%
Let $G$ be a $3$-regular graph on $n$ vertices with girth at least $(\log n)/10$ and edge expansion at least $0.01$ (such graphs are known to exist, see e.g., \cite{alon2021high}).
The weight on every edge in $G$ is $1$.
%Let $\dist_G(\cdot,\cdot)$ be the shortest-path distance metric in $G$. 
Denote $M = \floor{\sqrt{\log n}}$. 
We construct the set $T$ of terminals by the following lemma.


\begin{lemma} \label{lem:terminal}
We can efficiently compute a subset $T\subseteq V(G)$ of vertices, such that
    \begin{enumerate}
        \item for every pair $t,t'\in T$, $\dist_G(t,t')\ge M$; and
        \item for every vertex $v\in V(G)$, there are terminals $t_1,t_2 \in T$, such that $\dist_G(t_1,t_2)\le 10 M$ and the unique  $t_1$-$t_2$ shortest path in $G$ contains $v$.
    \end{enumerate}
\end{lemma}

\begin{proof}
We construct the set $T$ of terminals by an iterative algorithm. Initially, $T =\emptyset$, %Throughout the process, $T$ always satisfies the first condition.
and clearly it satisfies the first condition but not the second one. 
In each iteration, we take any vertex $v$ such that $T$ does not satisfy the second condition for $v$ (if there is no such vertex then we terminate the algorithm and return the current set $T$).
Consider the subgraph $R$ of $G$ induced by all vertices that are within distance $5M$ from $v$. As $G$ has girth $\Omega(\log n)>10M$, $R$ contains no cycles and is therefore a tree, and we denote by $\rset$ the collection of (three) subtrees of $R$ obtained by removing $v$. Observe that at most one subtree in $\tset$ contains a vertex in $T$, as otherwise the current set $T$ has satisfied the second condition for $v$, a contradiction. 
For each subtree in $\rset$ that does not contain a vertex of $T$, we pick an arbitrary vertex $v'$ in it with $\dist_G(v,v')=2M$, and add it to $T$. It is easy to verify that after augmenting $T$ in this way, the first condition still holds.
This completes the description of an iteration and also the algorithm. It is easy to see that the set $T$ grows after each iteration so the algorithm must terminate in at most $n$ iterations and return a set $T$ that satisfies both conditions.
\end{proof}

We show that any SPR solution $H$ of the instance $(G,T)$ constructed above has stretch $\Omega(\sqrt{\log n})$.
Note that this implies  \Cref{thm: main}, as the set $T$ of terminals constructed above has size at most $n$.
(Actually the size of $T$ is at least $n/3^{10M}$, so $\log |T|=\Theta(\log n)$.)
Let $\cset$ be the partitioning of $V(G)$ that generates $H$.
We denote $D = \log n/10^2$. We distinguish between the following cases. 

\subsubsection*{Case 1. Each cluster $C\in \cset$ has strong diameter at most $D$.}

Each cluster $C\in \cset$ contains at most $3^{D} < n/2$ vertices. As graph $G$ has edge-expansion at least $0.01$, the number of inter-cluster edges (edges with endpoints lying in different clusters in $\cset$) is at least $(1/2)\cdot \sum_{C\in \cset} 0.01\cdot |C|= n/200$. We use the following claims. 

\begin{claim}
\label{clm: touch}
For terminals $t,t'$ with $t\in C, t'\in C'$, if $\dist_{G}(t,t')\le 10^4M$ and the $t$-$t'$ shortest path in $G$ contains some vertex outside $C\cup C'$, then there is no edge in $G$ connecting $C$ and $C'$.
\end{claim}
\begin{proof}
Assume towards contradiction that some vertex $u$ on the $t$-$t'$ shortest path does not belong to $C\cup C'$, and there exist an edge $(v,v')$ with $v\in C$ and $v'\in C'$. Consider the union of 
\begin{itemize}
\item the $t$-$t'$ shortest path in $G$ (which has length at most $10^4M$);
\item the $t$-$v$ shortest path in $C$ (which has length at most $D$);
\item the $t'$-$v'$ shortest path in $C'$ (which has length at most $D$); and
\item the $(v,v')$ edge.
\end{itemize}
Clearly, they form a cycle (possibly non-simple). Via similar arguments as \Cref{obs: girth}, we can show that it contains a simple cycle (note that $u$ only participates in the first path), a contradiction as $10^4M+D+D+1<\gir(G)$.
\end{proof}

\iffalse
\begin{claim} \label{clm:different}
    For any vertex $u$ and $v$, if the distance between them is at most $2000M$ and they are in the same cluster $C$, then every point on the only shortest path between them is in the same cluster $C$.
\end{claim}

\begin{proof}
    Suppose there is some vertex on the path is not in $C$, then $u$ and $v$ is connected by a path of length at least $\log n /20$ in the cluster $C$ since $G$ has girth at least $\log n/10$. Consider any two vertex on that path whose distance is $2D$, the path is the only shortest path between them in $G$, thus the weak diameter of $C$ is at least $2D$, a contradiction.
\end{proof}

\fi

%The next claim show that there exist a path of length $1000M$ has at least $30M$ inter-cluster edges.

\begin{claim} \label{clm:path1}
There are two vertices $u,v\in V(G)$, such that $\dist_G(u,v)=10^4M$, and the unique $u$-$v$ shortest path in $G$ contains at least $50M$ inter-cluster edges.
\end{claim}

\begin{proof}
As $G$ is a $3$-regular graph with girth $(\log n)/10>2\cdot 10^4M$, the $10^4M$-neighborhood of each vertex $v$ is isomorphic (to the graph where $v$ is connected with three complete binary trees), and so each edge of $G$ appears in exactly the  same number of length-$10^4M$ paths in $G$. Therefore, some length-$10^4M$ path contains at least $(10^4\cdot M)\cdot (n/200)/n=50M$ inter-cluster edges. Clearly, this path is the unique shortest path between its endpoints, as $G$ has girth at least $2\cdot10^4M$.
\end{proof}

Consider the path $P$ given by \Cref{clm:path1} with endpoints $u,v$. From \Cref{lem:terminal}, there is some terminal $t\in T$ with $\dist_G(t,u)\le 5M$ and similarly there is some terminal $t'\in T$ with $\dist_G(t',v)\le 5M$, so 
$(10^4-10)M\le \dist_G(t,t')\le (10^4+10)M$.
From \Cref{obs: girth}, we get that the $t$-$t'$ shortest path $Q$ must lie entirely in the union of (i) the $t$-$u$ shortest path, (ii) the path $P$, and (iii) the $u'$-$t'$ shortest path, as otherwise they will create a cycle of length at most $3\cdot 10^4M<\gir(G)$.
As a corollary, $|E(Q)\setminus E(P)|\le 10M$.
%
It follows (from \Cref{clm:path1}) that $Q$ contains at least $40M$ inter-cluster edges.

%We prove that the distance between them in the minor is $\Omega(\log n)$. Note that for any path $P$ between $t_1$ and $t_2$ in the minor, there is a path (maybe not simple path) of the same length in the original graph such that the corresponding path in the minor is exactly $P$. Since the distance between $t_1$ and $t_2$ is at most $1010M$, the paths between them in $G$ are either contains every edge of the shortest path between them, or the length of the path is $\Omega(\log n)$. In the first case, the corresponding path in the minor contains at least $20M$ edges of length at least $M$, which means the length is at least $\Omega(M^2) = \Omega(\log n)$. Thus in both case, the path in the minor has length $\Omega(\log n)$, and this means the distortion of the minor is $\Omega(\log^{1/2} n)$.
%
Consider the $t$-$t'$ shortest path in $H$ and its image path $R$ in $G$. 
% 
As $\dist_G(t,t')\le (10^4+10)M$, from \Cref{obs: girth}, either $|R|\ge \gir(G)-(10^4+10)M\ge \Omega(\log n)$, or $Q\subseteq R$, which means $R$ contains at least $40M$ intercluster edges. 


\znote{to elaborate}
This means that the $t$-$t'$ shortest path in $H$ contains at least $40M$ edges with length at least $M$ each (as $\dist_H(t_1,t_2)\ge \dist_G(t_1,t_2)\ge M$ holds for all pairs $t_1,t_2$, from \Cref{lem:terminal}).
Therefore,
\[
\frac{\dist_{H}(t,t')}{\dist_{G}(t,t')}\ge \frac{40M\cdot M}{(10^4+10)M}=\Omega\Big(\sqrt{\log n}\Big).\]



\subsubsection*{Case 2. Some cluster $C\in \cset$ has weak diameter greater than $D$.}

Let $t^*$ be the center of $C$.
Let $v$ be a vertex in $C$ with $\dist_{G}(t,t')\ge D/2$. From \Cref{lem:terminal}, there are terminals $t_1,t_2$ such that $\dist_G(t_1,t_2)\le 10 M$ and the unique $t_1$-$t_2$ shortest path in $G$ contains $v$. Note that $\dist_G(t^*,t_1),\dist_G(t^*,t_2)\ge D/2-10M$.
Consider the $t_1$-$t_2$ shortest path in $H$. If this path contains $t^*$, then it has length at least $D-20M = \Omega(\log n)$. 

\znote{incorrect here} Otherwise, consider its image path $R$ and the $t_1$-$t_2$ shortest path $P$, From \Cref{obs: girth}, its image path has length at least $\gir(G)-10M\ge \Omega(\log n)$, and from \Cref{obs: minor dist} it follows that $\dist_{H}(t,t')=\Omega(\log n)$.
Altogether,
\[
\frac{\dist_{H}(t,t')}{\dist_{G}(t,t')}\ge \frac{\Omega(\log n)}{10M}=\Omega\Big(\sqrt{\log n}\Big).\]



==> headers.tex <==
\iffalse
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{shapes}
\usetikzlibrary{backgrounds}
\usetikzlibrary{positioning}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{patterns}
\usetikzlibrary{calc}
\usetikzlibrary{fit}
\usetikzlibrary{snakes}
\usetikzlibrary{shadows.blur}
\usetikzlibrary{petri,decorations.markings}
\fi

\renewcommand{\top}{T}

\RequirePackage{silence}
\WarningFilter{remreset}{The remreset package}
\usepackage{fancybox}
\usepackage{enumitem}

\setlistdepth{9}

\newlist{myEnumerate}{enumerate}{5}
\setlist[myEnumerate,1]{label=\arabic*.}
\setlist[myEnumerate,2]{label=(\alph*)}
\setlist[myEnumerate,3]{label=\roman*.}
\setlist[myEnumerate,4]{label=\Alph*.}
\setlist[myEnumerate,5]{label=\Roman*.}
%\setlist[myEnumerate,6]{label=(\arabic*)}
%\setlist[myEnumerate,7]{label=(\Roman*)}
%\setlist[myEnumerate,8]{label=(\Alph*)}
%\setlist[myEnumerate,9]{label=(\roman*)}

%\usepackage{kbordermatrix}
%\renewcommand{\kbldelim}{(}% Left delimiter
%\renewcommand{\kbrdelim}{)}% Right delimiter
\usepackage{blkarray}
\usepackage{array}
%\newcolumntype{x}[1]{>{\centering\arraybackslash\hspace{0pt}}p{#1}}
\newcolumntype{x}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand{\mLabel}[1]{\mbox{$\scriptstyle{#1}$}}

\usepackage{stackengine}
\newcommand\xrowht[2][0]{\addstackgap[.5\dimexpr#2\relax]{\vphantom{#1}}}
%\usepackage{enumerate}

\newcommand{\gy}{G_{\sigma_n}^{\mathrm{yes}}}
\newcommand{\gn}{G_{\sigma_n}^{\mathrm{no}}}
\newcommand{\dtv}{D_{\mathrm{TV}}}

\usepackage{amsmath,amsfonts,amssymb,amsthm,bm}
\usepackage{color,xcolor}
%\usepackage[colorlinks=true]{hyperref}
\usepackage{nameref}
\definecolor{azure}{rgb}{0.0, 0.5, 1.0}
\definecolor{ForestGreen}{rgb}{0.1333,0.5451,0.1333}
\definecolor{myred}{rgb}{0.8,0.25,0.25}
\definecolor{DarkRed}{rgb}{0.7, 0.0, 0.0}
\usepackage[linktocpage=true, pagebackref=true,colorlinks, linkcolor=DarkRed,citecolor=ForestGreen, bookmarks,bookmarksopen,bookmarksnumbered]{hyperref}

\usepackage[noabbrev,nameinlink]{cleveref}
\crefname{property}{property}{Property}
\creflabelformat{property}{(#1)#2#3}
\crefname{equation}{eq}{Eq}
\creflabelformat{equation}{(#1)#2#3}
\usepackage[procnumbered,ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{amsfonts}
\usepackage{thm-restate}
\usepackage{blindtext}
\usepackage{thm-restate}

\iffalse
\textheight 8.5in
\topmargin -0.2in
\oddsidemargin 0.20in
\textwidth 6.3in
\fi

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemm}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{warning}[theorem]{Warning}

\theoremstyle{definition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{assumption}[lemm]{Assumption}
\newtheorem{definition}[lemm]{Definition}
\newtheorem{remark}[lemm]{Remark}
\newtheorem{problem}{Problem}


\newcommand{\highlight}[1]{\colorbox{yellow}{#1}}


\newenvironment{fminipage}%
  {\begin{Sbox}\begin{minipage}}%
  {\end{minipage}\end{Sbox}\fbox{\TheSbox}}

\newenvironment{algbox}[0]{%\vskip 0.2in
\noindent
%\begin{figure}
  \begin{center}
\begin{fminipage}{1\textwidth}%{6.3in}
}{
\end{fminipage}
\end{center}
%\end{figure}
%\vskip 0.2in
}

%\newenvironment{probbox}[0]{\vskip 0.1in
%%\noindent 
%  \begin{center}
%        \begin{fminipage}{5.7in}
%}{
%\end{fminipage}
%\end{center}
%\vskip 0.1in
%}

% Algorithm2e
\DontPrintSemicolon
\SetKw{KwAnd}{and}
\SetProcNameSty{textsc}
\SetFuncSty{textsc}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\def\dr{\mathrm{d}}

\def\pleq{\preceq} %curlyeq}
\def\pgeq{\succeq} %curlyeq}
\def\pge{\succ}
\def\ple{\prec}
\def\sc{\textsc{SC}}

\newcommand\AGM{\textsc{UnweightedCutSparsify}}
\newcommand\WGM{\textsc{WeightedCutSparsify}}
\newcommand\WL{\textsc{WeightedEdgeSampler}}

\newcommand\HVS{\textsc{HeavyEdgeSketch}}
\newcommand\HVR{\textsc{HeavyEdgeRecovery}}

\newcommand\WSS{\textsc{SpectralSketch}}
\newcommand\WSR{\textsc{SpectralRecovery}}

\newcommand\SQS{\textsc{SquareSketch}}
\newcommand\SQR{\textsc{SquareRecovery}}

\newcommand\SVS{\textsc{SquareHeavySketch}}
\newcommand\SVR{\textsc{SquareHeavyRecovery}}

\newcommand\SSQ{S^{\mathrm{sq}}}
\newcommand\SSS{S^{\mathrm{ss}}}
\newcommand\SHV{S^{\mathrm{hv}}}
\newcommand\SSV{S^{\mathrm{sqh}}}

\def\detp{\det\nolimits_{+}}
\def\detb#1{\det\nolimits_{#1}}
\def\detz{\det\nolimits_{(0,\zeta]}}
\def\detzz{\det\nolimits_{(0,\zeta']}}
\def\detl{\det\nolimits_{\ell}}
\def\detll{\det\nolimits_{\ell'}}
\def\detn{\det\nolimits}

\def\dr{\mathrm{d}}

\def\Approx#1{\approx_{#1}}

\def\Span#1{\textbf{Span}\left(#1  \right)}
\def\bvec#1{{\mbox{\boldmath $#1$}}}


\def\prob#1#2{\mathrm{Pr}_{#1}\left[ #2 \right]}
\def\pr#1{\mathrm{Pr}\left[ #1 \right]}
\def\pvec#1#2{\vec{\mbox{P}}^{#1}\left[ #2 \right]}
\def\expec#1#2{{\mathbb{E}}_{#1}\left[ #2 \right]}
\def\ex#1{{\mathbb{E}}\left[ #1 \right]}
\def\var#1{\mbox{\bf Var}\left[ #1 \right]}
\newcommand{\E}{\mbox{{\bf E}}}

\def\defeq{\stackrel{\mathrm{def}}{=}}
\def\setof#1{\left\{#1  \right\}}
\def\sizeof#1{\left|#1  \right|}
\def\card#1{\left| #1 \right|}
\def\deg{\textrm{deg}}




\def\floor#1{\left\lfloor #1 \right\rfloor}
\def\ceil#1{\left\lceil #1 \right\rceil}

\def\dim#1{\mathrm{dim} (#1)}
\def\sgn#1{\mathrm{sgn} (#1)}

\def\union{\cup}
\def\intersect{\cap}
\def\Union{\bigcup}
\def\Intersect{\bigcap}

\def\eps{\epsilon}

\def\abs#1{\left|#1  \right|}

\def\rank#1{\mathrm{rank} \left(#1 \right)}
\def\trace#1{\mathrm{Tr} \left(#1 \right)}
\def\norm#1{\left\| #1 \right\|}
\def\normm#1{\lambdamax\kh{#1}}
\def\smallnorm#1{\| #1 \|}

\def\comp#1{#1^\complement}

\def\Acal{\mathcal{A}}
\def\Ncal{\mathcal{N}}
\def\Rcal{\mathcal{R}}
\def\Bcal{\mathcal{B}}
\def\Ccal{\mathcal{C}}
\def\Dcal{\mathcal{D}}
\def\Ecal{\mathcal{E}}
\def\Fcal{\mathcal{F}}
\def\Mcal{\mathcal{M}}
\def\Xcal{\mathcal{X}}
\def\Ftil{\tilde{F}}
\def\Htil{\tilde{H}}
\def\Ztil{\tilde{Z}}
\def\Ltil{\tilde{L}}
\def\wtil{\tilde{w}}
\def\Fcaltil{\tilde{\mathcal{F}}}
\def\Lambdatil{\tilde{\Lambda}}
\def\Hcal{\mathcal{H}}
\def\Ical{\mathcal{I}}
\def\Itil{\tilde{{I}}}
\def\Gcal{\mathcal{G}}
\def\Rcal{\mathcal{R}}
\def\phitil{\tilde{\phi}}
\def\Ucal{\mathcal{U}}
\def\Vcal{\mathcal{V}}
\def\Lcal{\mathcal{L}}
\def\Scal{\mathcal{S}}
\newcommand\Tcal{\mathcal{T}}
%\newcommand\Ucal{\mathcal{U}}
\newcommand\Pcal{\mathcal{P}}

\newcommand\xtil{\tilde{x}}
\newcommand\Gtil{\tilde{G}}

\newcommand\pth{\mathfrak{p}}


\newcommand\Ppsi{\boldsymbol{\mathit{\Psi}}}
\newcommand\PPsi{\boldsymbol{\mathit{\Psi}}}
\newcommand\ppsi{\boldsymbol{\mathit{\psi}}}
\newcommand\pphi{\boldsymbol{\mathit{\phi}}}
\newcommand\Llambda{\boldsymbol{\mathit{\Lambda}}}
\newcommand\PPi{\boldsymbol{\Pi}}

%\newcommand\ppi{\boldsymbol{\pi}}
\newcommand\ppi{\vec{\pi}}
\newcommand\cchi{\boldsymbol{\chi}}
\newcommand\aalpha{\boldsymbol{\alpha}}
\newcommand\bbeta{\boldsymbol{\beta}}
\newcommand\ggamma{\boldsymbol{\gamma}}
\newcommand\ddelta{\boldsymbol{\delta}}

\newcommand\er{R_{\mathrm{eff}}}
\newcommand\ccc{C_{\mathrm{CC}}}
\newcommand\ci{C_{\mathrm{I}}}


\def\lev{\mathtt{lev}}
\def\aa{\pmb{\mathit{a}}}
\newcommand\bb{\boldsymbol{\mathit{b}}}
%\newcommand\cc{\boldsymbol{\mathit{c}}}
\newcommand\cc{\boldsymbol{\mathit{c}}}
\newcommand\dd{\boldsymbol{\mathit{d}}}
\newcommand\ee{\boldsymbol{\mathit{e}}}
\newcommand\ff{\boldsymbol{\mathit{f}}}
%\renewcommand\gg{\boldsymbol{\mathit{g}}}
\newcommand\ii{\boldsymbol{\mathit{i}}}
\newcommand\jj{\boldsymbol{\mathit{j}}}
\newcommand\kk{\boldsymbol{\mathit{k}}}
%\renewcommand\ll{\boldsymbol{\mathit{\ell}}}
\newcommand\pp{\boldsymbol{\mathit{p}}}
\newcommand{\ttau}{{\boldsymbol{\mathit{\tau}}}}
\newcommand\qq{\boldsymbol{\mathit{q}}}
\newcommand\bs{\boldsymbol{\mathit{s}}}
%\newcommand\nn{\boldsymbol{\mathit{n}}}
\newcommand\nn{\vec{n}}
\newcommand\mm{\vec{m}}
\newcommand\rr{\boldsymbol{\mathit{r}}}
\newcommand\rrh{{\boldsymbol{\widehat{\mathit{{r}}}}}}
\renewcommand\dh{\widehat{d}}
\newcommand\wh{\widehat{w}}
\renewcommand\ss{\boldsymbol{\mathit{s}}}
\def\tt{\boldsymbol{\mathit{t}}}
\newcommand\uu{\boldsymbol{\mathit{u}}}
\newcommand\vv{\boldsymbol{\mathit{v}}}
\newcommand\ww{\boldsymbol{\mathit{w}}}
\newcommand\yy{\boldsymbol{\mathit{y}}}
\newcommand\zz{\boldsymbol{\mathit{z}}}
\newcommand\xx{\boldsymbol{\mathit{x}}}
\newcommand\xxbar{\overline{\boldsymbol{\mathit{x}}}}

\newcommand\dbar{d_{\mathrm{avg}}}

\renewcommand\AA{\boldsymbol{\mathit{A}}}
\newcommand\BB{\boldsymbol{\mathit{B}}}
\newcommand\CC{\boldsymbol{\mathit{C}}}
\newcommand\DD{\boldsymbol{\mathit{D}}}
\newcommand\EE{\boldsymbol{\mathit{E}}}
\newcommand\GG{\boldsymbol{\mathit{G}}}
\newcommand\II{\boldsymbol{\mathit{I}}}
\newcommand\JJ{\boldsymbol{\mathit{J}}}
\newcommand\KK{\boldsymbol{\mathit{K}}}
\newcommand\NN{\boldsymbol{\mathit{N}}}
\newcommand\MM{\mathrm{\textsf{M}}}
\newcommand\LL{\boldsymbol{\mathit{L}}}
\newcommand\HH{\boldsymbol{\mathit{H}}}
\newcommand\PP{\boldsymbol{\mathit{P}}}
\newcommand\QQ{\boldsymbol{\mathit{Q}}}
\newcommand\RR{\boldsymbol{\mathit{R}}}
\renewcommand\SS{\boldsymbol{\mathit{S}}}
\newcommand\TT{\boldsymbol{\mathit{T}}}
\newcommand\UU{\boldsymbol{\mathit{U}}}
\newcommand\WW{\boldsymbol{\mathit{W}}}
\newcommand\VV{\boldsymbol{\mathit{V}}}
\newcommand\XX{\boldsymbol{\mathit{X}}}
\newcommand\YY{\boldsymbol{\mathit{Y}}}

\def\sfy{{\sf Yes} }
\def\sfn{{\sf No} }
\newcommand\nnz{\mathrm{nnz}}
\newcommand\tv{\mathrm{TV}}
\newcommand\yes{\mathrm{yes}} % {\mathrm{yes}}
\newcommand\no{\mathrm{no}}

\newcommand\shat{\hat{s}}
\newcommand\ftil{\tilde{f}}
\newcommand\lambdatil{\tilde{\lambda}}
\newcommand\Ntil{\tilde{N}}
\newcommand\dtil{\tilde{d}}
\newcommand\Dtil{\tilde{D}}
\newcommand\MMtil{\boldsymbol{\mathit{\tilde{M}}}}
\newcommand\AAtilde{\boldsymbol{\mathit{\tilde{A}}}}
\newcommand\LLtil{\boldsymbol{\mathit{\tilde{L}}}}
\newcommand\MMtilde{\boldsymbol{\mathit{\tilde{M}}}}

\newcommand\AAn{\boldsymbol{\mathcal{A}}}
\newcommand\ZZ{\boldsymbol{\mathit{Z}}}

\newcommand\ZZtil{\widetilde{\boldsymbol{\mathit{Z}}}}

\newcommand\AAhat{\boldsymbol{\widehat{\mathit{A}}}}
\newcommand\AAapprox{\boldsymbol{\widetilde{\mathit{A}}}}
\newcommand\DDhat{\boldsymbol{\widehat{\mathit{D}}}}
\newcommand\DDapprox{\boldsymbol{\widetilde{\mathit{D}}}}
\newcommand\LLhat{\boldsymbol{\widehat{\mathit{L}}}}
\newcommand\LLapprox{\boldsymbol{\widetilde{\mathit{L}}}}
\newcommand\MMhat{\boldsymbol{\widehat{\mathit{M}}}}
\newcommand\MMapprox{\boldsymbol{\widetilde{\mathit{M}}}}
\newcommand\ZZhat{\boldsymbol{\widehat{\mathit{Z}}}}

\newcommand\AAtil{\boldsymbol{\widetilde{\mathit{A}}}}
\newcommand\DDtil{\boldsymbol{\widetilde{\mathit{D}}}}


\newcommand\bbtil{\boldsymbol{\tilde{\mathit{b}}}}
\newcommand\xxtil{\boldsymbol{\tilde{\mathit{x}}}}


\newcommand\Otil{\tilde{O}}
\newcommand\otil{\tilde{o}}
\newcommand\Ktil{\tilde{K}}
\newcommand\Thetatil{\tilde{\Theta}}
\newcommand\Omegatil{\tilde{\Omega}}

\newcommand\xhat{\boldsymbol{\hat{\mathit{x}}}}
\newcommand\uhat{{\hat{{u}}}}
\newcommand\vhat{{\hat{{v}}}}
\newcommand\what{{\hat{{w}}}}

\newcommand\fbf{\mathbf{f}}

\newcommand\Ghat{{\widehat{{G}}}}

\newcommand{\sym}[1]{\mathrm{sym} (#1)}

\newcommand{\zero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\diag}{\textsc{diag}}
\newcommand\LLs{\boldsymbol{\mathit{L}_s}}
\newcommand\SSi{\boldsymbol{\Sigma}}

\newcommand\dila{\mathtt{dila}}
\newcommand\cont{\mathtt{ctrc}}
\newcommand\area{\mathtt{area}}
\newcommand\vol{\mathsf{cost}}
\newcommand\scolon{\hspace{-2.5pt}:\hspace{-1.5pt}}

\newcommand\DS{\textsc{DetScheduling}}
\newcommand\DP{\textsc{DPScheduling}}
\newcommand\RI{\textsc{Rounded}}
\newcommand\PTAS{\textsc{PoiScheduling}}
\newcommand\ILP{\textsc{ILPScheduling}}
\newcommand\IP{\textsc{ILP}}
\newcommand\CHEBY{\textsc{ChebySolve}}
\newcommand\HARGD{\textsc{AlmostRegularDecomp}}
\newcommand\HED{\textsc{ExpanderDecomp}}
\newcommand\WAM{\textsc{Whack-a-mole-I}}
\newcommand\WTM{\textsc{Whack-a-mole-II}}
\newcommand\WAME{\textsc{Whack-a-mole-Exp}}

\newcommand\la{\leftarrow}

\newcommand\TEST{\textsc{Traps?}}
\newcommand\MBSWB{\textsc{NoisyBinarySearchRW}}

\newcommand\IR{\textsc{Sparisfy}}
\newcommand\SP{\textsc{SampleWR}}

\newcommand\SC{\mathrm{SC}}
\newcommand\SCN{\mathrm{SC}_n}

\newcommand{\sd}{\geq_{\mathrm{sd}}}

\newcommand{\todo}[1]{{\bf \color{red} TODO: #1}}
\newcommand{\hl}[1]{{\bf \color{orange} Huan: #1}}
%\newcommand{\yhy}[1]{{\color{blue} #1}}
%\newcommand{\zzz}[1]{{\bf \color{green} Zhongzhi: #1}}
%\newcommand{\sep}[1]{{\color{blue}#1}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\poi}[1]{\mathrm{Poi}\left(#1\right)}

\newcommand{\kh}[1]{\left(#1\right)}

\newcommand{\ip}[2]{\left\langle#1,#2\right\rangle}

\newcommand{\wmax}{w_{\max}}
\newcommand{\wmin}{w_{\min}}

\newcommand{\lambdamin}{\lambda_{\mathrm{min}}}
\newcommand{\lambdamax}{\lambda_{\mathrm{max}}}

\newcommand{\poly}{\mathrm{poly}}
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\ade}[1]{{\color{blue}#1}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\by}{\mathbf{y}}

\newcommand{\dmin}{d_{\mathrm{min}}}

